Out-of-Distribution Detection via Deep Multi-Comprehension Ensemble

Recent research underscores the pivotal role of the Out-of-Distribution (OOD) feature representation field scale in determining the efficacy of models in OOD detection. Consequently, the adoption of model ensembles has emerged as a prominent strategy to augment this feature representation field, capitalizing on anticipated model diversity. However, our introduction of novel qualitative and quantitative model ensemble evaluation methods, specifically Loss Basin/Barrier Visualization and the Self-Coupling Index, reveals a critical drawback in existing ensemble methods. We find that these methods incorporate weights that are affine-transformable, exhibiting limited variability and thus failing to achieve the desired diversity in feature representation. To address this limitation, we elevate the dimensions of traditional model ensembles, incorporating various factors such as different weight initializations, data holdout, etc., into distinct supervision tasks. This innovative approach, termed Multi-Comprehension (MC) Ensemble, leverages diverse training tasks to generate distinct comprehensions of the data and labels, thereby extending the feature representation field. Our experimental results demonstrate the superior performance of the MC Ensemble strategy in OOD detection compared to both the naive Deep Ensemble method and a standalone model of comparable size. This underscores the effectiveness of our proposed approach in enhancing the model's capability to detect instances outside its training distribution.

==> _hist/0_Abstract_v1.tex <==
\begin{abstract}

The detection of out-of-distribution (OOD) samples is a critical task in the inference stage of machine learning models, particularly in domains where security is of utmost importance. OOD detection is aimed at identifying samples that do not belong to the training distribution, which can help prevent potential security breaches or other undesired consequences. 
    Previous studies have attempted to improve the performance of OOD detection by constructing ensemble models that leverage the differences between initialization or training data.
However, we observe that the previous ensemble model can provide only limited diversity when examining the coupling matrix of the penultimate layer feature representation between different models, as well as the mode connectivity between models. To overcome this limitation, we propose a new ensemble strategy, Multi-Comprehensive Ensemble (MC Ensemble), which employs multiple training criteria to decrease the Self-Coupling Index of samples between each individual model to improve diversity.
    The MC Ensemble approach is scalable and distillable, and it can be combined with any other post-hoc OOD detection scoring metrics. 
        In experiments, we demonstrate the superior performance of the MC Ensemble strategy in the OOD detection task compared to the naive Deep Ensemble model and a single model of the same size.

\end{abstract}

==> _hist/1_Introduction.tex <==
\section{Introduction}
State-of-the-art neural network models tend to make over-confident predictions, because they are trained and generalized in a static and closed world. 
    That is, an assumption that the distribution of test samples will be same as training samples. 
    In the open world, however, the case does not necessarily conform to the above assumption because of out-of-distribution~(OOD) samples coming from unreliable data source or adversarial attack. 
%    For example, when you feed an image of a flower into an animal classifier, you don't expect the classifier to give a highly confident answer, but it does. 
Based on the reliability and safety concerns, it is critical to ascertain whether the input is out-of-distribution.
    Enormous research efforts have been put on the OOD detection as well as uncertainty estimation.~\cite{lakshminarayanan2017simple,liang2017enhancing,hendrycks2019using,ren2019likelihood,huang2021importance,liu2020energy}

In practice, researchers propose employing an ensemble of neural networks, that combines multiple independent models to improve model predictive robustness against OOD samples~\cite{lakshminarayanan2017simple,zaidi2021neural,malinin2019ensemble,kariyappa2021protecting,li2021k}. 
    Inspired by Bagging~\cite{breiman1996bagging}, \emph{Deep Ensembles}~\cite{lakshminarayanan2017simple} which take the average of posterior probability generated by the same models with different initialization is proposed with the advantages of being pervasive and scalable. 
%However, not everyone agree with the necessity of ensemble models. 
   % \cite{miller2021accuracy} points out that model's out-of-distribution performance is strongly correlated with in-distribution performance, which hints that maybe Deep Ensembles' OOD detection performance do not have a direct causality with ensemble itself.
  %  Furthermore, \cite{abedeep} directly denies the claim of ensemble methods that feature diversity contributes to the OOD detection performance by validating a single model with similar scale. 
%But the question is: \emph{Is diversity really not contributing anything?}
%这一段的claim不太对，之前工作否认的是OOD generalization的能力，detection能力仍然有待考察。后续可以先从这个角度入手

%We first review that from which perspectives have previous ensemble works claimed its own diversity. 
   % Deep Ensembles~\cite{lakshminarayanan2017simple} defines its diversity as that neural networks with different weight initialization tends to convergence to different suboptimal solutions after training, and therefore, they will generate diversified feature representations. 
  %  \cite{li2021k}~and~\cite{vyas2018out} adopt $k$~fold cross validation and class-level leave out respectively, and claim their diversity from training data perspective. 
%However, as shown in Figure~%\ref{} 还没画
%, after training towards the one-hot label representation, models with different weight initialization tend to generate output feature representation with diversity reflected in relative position with regard to labels, but not in density. 
   % That means, there are mappings whose norm is close to $1$ can fit the transformation among different feature representations with regard to labels.
   % The deep ensembles, therefore, fail to extract a diversified posterior that really helps to distinguish the OOD samples. 
%After counteracting the effect of weight initialization, the data diversity introduced by $k$~fold cross validation and leave out still do not have strong diversity since most of the data are overlapped, and thus the densities are similar. 
%So, the reason why previous ensemble-based method fails to significantly superior to single-larger model may attribute to that the diversity along with ensemble is not strong enough.
%这个diversity怎么度量？

%这里开始写我们的从不同训练方式出发的ensemble方法，先从ssl，contrastive分别的优势说起，最终提出enesmble

%在下一段简单的回归softmax scoring的问题，回顾mahalanobis distance，knn等scoring更有效，提出reunify with scoring metric的ensemble。

%实验的小结，之后写

%Contribution：1.提出之前ensemble还存在的缺陷。 2.Diversity：training策略的ensemble。 3.Reunify：scoring metric的ensemble。

==> _hist/1_Introduction_v2.tex <==
\section{Introduction}
State-of-the-art neural network models tend to make over-confident predictions, because they are trained and generalized in a static and closed world. 
    That is, an assumption that the distribution of test samples will be same as training samples. 
    In the open world, however, the case does not necessarily conform to the above assumption because of out-of-distribution~(OOD) samples coming from unreliable data source or adversarial attack. 
%    For example, when you feed an image of a flower into an animal classifier, you don't expect the classifier to give a highly confident answer, but it does. 
Based on the reliability and safety concerns, it is critical to ascertain whether the input is out-of-distribution.
    Enormous research efforts have been put on the OOD detection as well as uncertainty estimation.~\cite{lakshminarayanan2017simple,liang2017enhancing,hendrycks2019using,ren2019likelihood,huang2021importance,liu2020energy}

In practice, researchers propose employing an ensemble of neural networks, that combines multiple independent models to improve model predictive robustness against OOD samples~\cite{lakshminarayanan2017simple,zaidi2021neural,malinin2019ensemble,kariyappa2021protecting,li2021kfolden}. 
    Inspired by Bagging~\cite{breiman1996bagging}, \emph{Deep Ensembles}~\cite{lakshminarayanan2017simple} which take the average of posterior probability generated by the same models with different initialization is proposed with the advantages of being pervasive and scalable.
However, ensembles face to such two problems: The first is, due to the intrinsic simplicity bias~\cite{pagliardini2022agree} of the neural networks, the individuals in an ensemble tend to show a strong consistency. That is, although with different initialization and training samples, the models mapping the input samples into similar posterior after training with same criterion. The second is, although ensembles work well, their computation overhead fold increase w.r.t. the number of ensemble members, which limits the deployment on real-world edge device with limited sources and unsatisfy the real time demands.
%Ensemble 的两个问题：simplicity bias导致的趋同性，although scalable，但是inference开销是成倍增加

We experimentally and theoretically point out that networks based on the same criterion but with different initializations, after being trained by stochastic gradient descent~(SGD), differ weakly in their encoding of the same input in the representation space. 
    The weakness of this difference is due to the fact that, given the criterion, the neural network loss landscapes approximation considering various possible permutation symmetries contains only one loss basin.～\cite{ainsworth2023git}. 
        Thus, to some extent, networks trained on the same distributed dataset according to the same criterion based on SGD are highly correlated (or even equivalent).
    This weak difference prevents the ensemble from achieving the expected results on the OOD detection task.

By measuring the differences in the distribution of different models' encoding of the same dataset on the penultimate layer of features (commonly used to calculate OOD scores) through the Wassernstein distance~\cite{vallender1974calculation} and its corresponding sample coupling matrix, we found that training criterion would be an important factor in diversity.
    To further substantiate our findings, we also evaluated the loss barrier between models trained on different criteria. 
        Our results demonstrate that the models trained using different criteria exhibit a more significant loss barrier, implying that the models do not have the same loss landscapes. Consequently, these models display greater dissimilarities.

Based on the above assumptions and findings, we designed a new ensemble scheme which integrates models based on different criterion training with the same structure and the same training data. Experiments show that this is a better ensemble scheme compared to other schemes such as k-fold ensemble

\textbf{Contributions.} We make the following contributions:

\begin{itemize}
    \item We reveal that the previous ensembles' lack of success in detecting OOD samples can be attributed to the inadequate degree of diversity among models trained using the same criterion.
    \item We design a feature-level ensemble scheme that exploits the diversity of models based on different criterions, making the OOD samples more distant from the class center in average.
    \item We propose to obtain more easily deployable OOD-sensitive models by distillation with ensemble for feature alignment.
\end{itemize}

%Consider OOD detector as a 0-1 classifier, which contains a feature encoder shared with the main task and a scoring metric determining whether an input is OOD. 

%The prevailing approach in OOD detection involves a detector that consists of a feature encoder and a scoring metric. 
%    The feature encoder, which is shared with the main task, encodes the input into the penultimate layer feature representation space. 
 %   While the scoring metric (such as Mahalanobis Distance~\cite{lee2018simple}, energy-score~\cite{liu2020energy}, and kNN-score~\cite{sun2022out}) determines whether an input sample is OOD based on the features extracted at the penultimate layer.
%Usually a neural network can be divided into two parts in the inference phase, the encoder $g(\codt)$ that encodes the input into the representation space and the functional projection head $h(\cdot)$ that is based on the FEATURE representation.
%The reason why an ensemble works in OOD detection is based on the following bias-variance decomposition:
%\begin{equation}
 %   Error(C) = \sum_{x}P(x)(bias_{ensemble}^2+\frac{1}{M^2}\sum_{i=1}{M}variance(f_i)+\frac{1}{M(M-1)}\sum_{i \neq j}{M}cov(f_i,f_j)
%\end{equation}

%\sum_{y \in Y}[P(Y_F=y|x)-\frac{1}{M}\sum_{i=1}^MP(Y_{H_i}=y|x)]^2
%The diversity of individuals in the ensemble makes each individual produce a disagreement on the OOD sample.\cite{pagliardini2022agree}. 
%The ensemble model makes a high uncertainty prediction for the OOD sample due to the disagreement, while giving a consistent prediction for the in-distribution (ID) sample. 
   % This requires the assumption that different individual models understand the sample from different perspectives. 
     %   There are many ways of such understanding; in the case of images, it includes color, local shape, texture, background, and other understandable perspectives. 
   % The simplicity bias means that the model will choose a simpler perspective if it provides similar or better performance compared to a more complex one.
     
%However, not everyone agree with the necessity of ensemble models. 
   % \cite{miller2021accuracy} points out that model's out-of-distribution performance is strongly correlated with in-distribution performance, which hints that maybe Deep Ensembles' OOD detection performance do not have a direct causality with ensemble itself.
  %  Furthermore, \cite{abedeep} directly denies the claim of ensemble methods that feature diversity contributes to the OOD detection performance by validating a single model with similar scale. 
%But the question is: \emph{Is diversity really not contributing anything?}
%这一段的claim不太对，之前工作否认的是OOD generalization的能力，detection能力仍然有待考察。后续可以先从这个角度入手

%We first review that from which perspectives have previous ensemble works claimed its own diversity. 
   % Deep Ensembles~\cite{lakshminarayanan2017simple} defines its diversity as that neural networks with different weight initialization tends to convergence to different suboptimal solutions after training, and therefore, they will generate diversified feature representations. 
  %  \cite{li2021k}~and~\cite{vyas2018out} adopt $k$~fold cross validation and class-level leave out respectively, and claim their diversity from training data perspective. 
%However, as shown in Figure~%\ref{} 还没画
%, after training towards the one-hot label representation, models with different weight initialization tend to generate output feature representation with diversity reflected in relative position with regard to labels, but not in density. 
   % That means, there are mappings whose norm is close to $1$ can fit the transformation among different feature representations with regard to labels.
   % The deep ensembles, therefore, fail to extract a diversified posterior that really helps to distinguish the OOD samples. 
%After counteracting the effect of weight initialization, the data diversity introduced by $k$~fold cross validation and leave out still do not have strong diversity since most of the data are overlapped, and thus the densities are similar. 
%So, the reason why previous ensemble-based method fails to significantly superior to single-larger model may attribute to that the diversity along with ensemble is not strong enough.
%这个diversity怎么度量？

%这里开始写我们的从不同训练方式出发的ensemble方法，先从ssl，contrastive分别的优势说起，最终提出enesmble

%在下一段简单的回归softmax scoring的问题，回顾mahalanobis distance，knn等scoring更有效，提出reunify with scoring metric的ensemble。

%实验的小结，之后写

%Contribution：1.提出之前ensemble还存在的缺陷。 2.Diversity：training策略的ensemble。 3.Reunify：scoring metric的ensemble。

\begin{figure}[t]
    \centering
    \includegraphics{_fig/coupling-matrix.pdf}
    \caption{Coupling matrix of the OOD sample penultimate layer feature distribution's Wasserstein distance of the two networks. Highlighting on the diagonal indicates that the two sets of feature representations are aligned regarding to the samples, which indicates that there is little variability in the two distributions. SupCE = Supervised Cross  Entropy loss, SupCon = Supervised Contrastive loss~\cite{khosla2020supervised}, SimCLR = Simple Contrastive Learning Representation~\cite{chen2020simple}
    \label{fig:my_label}
\end{figure}

==> _hist/1_Introduction_v2_polished_by_ChatGPT.tex <==
\section{Introduction}
State-of-the-art neural network models often exhibit overconfidence in their predictions due to their training and generalization in a static and closed environment. 
    Specifically, these models assume that the distribution of test samples is identical to that of the training samples. 
        However, in the open world, this assumption may not hold, as out-of-distribution (OOD) samples can arise from unreliable data sources or adversarial attacks. 
            Such OOD samples can introduce significant challenges to the generalization performance of these models.
Due to concerns related to reliability and safety, it is crucial to identify when input data is OOD. 
    Significant research efforts have been devoted to the detection of OOD samples~\cite{liang2018enhancing,hendrycks2019using,ren2019likelihood,huang2021importance,liu2020energy}, as well as the estimation of uncertainty~\cite{lakshminarayanan2017simple} in networks.

In practice, researchers have proposed employing an ensemble of neural networks, which involves combining multiple independent models to enhance the robustness of model predictions against OOD samples~\cite{lakshminarayanan2017simple,zaidi2021neural,Malinin2020Ensemble,kariyappa2021protecting,li2021kfolden,xue2022boosting}. 
Inspired by the Bagging~\cite{breiman1996bagging} method, researchers have proposed \emph{Deep Ensembles}~\cite{lakshminarayanan2017simple}, which calculate the average of the posterior probabilities generated by multiple models with different initializations. 
    This approach offers the advantages of being both pervasive and scalable. However, ensembles face two main challenges. The first issue is related to the intrinsic simplicity bias~\cite{pagliardini2022agree} of neural networks. 
        Specifically, the members of an ensemble tend to exhibit strong consistency, meaning that even with different initializations and training samples, the resulting models map input samples to similar posterior distributions after training with the same criterion.
            The second issue with ensembles is that their computational overhead increases significantly with the number of ensemble members, which can limit their deployment on real-world edge devices with limited resources and real-time requirements. Although ensembles are effective, this overhead can make them unsuitable for certain applications.


%Our study, conducted through a combination of experimental and theoretical analyses, 
Experimentally and theoretically, we reveals that neural networks trained using the same criterion but with different initializations and stochastic gradient descent (SGD) display only weak differences in their encoding of the same input in the representation space.
    This phenomenon arises from the hypothesis that, given the training criterion, the approximation of the neural network loss landscapes, accounting for various possible permutation symmetries, comprises only a single loss basin. \cite{ainsworth2023git}
        Consequently, networks trained on the same distributed dataset with the same criterion using SGD are highly correlated or even functionally equivalent to a considerable extent. 
Nonetheless, this marginal disparity impedes the ensemble's ability to achieve anticipated outcomes in detecting OOD samples.

 In this paper, we employed the Wasserstein distance and its corresponding sample coupling matrix to quantify the differences in the distribution of the same dataset's encoding by various models in the penultimate layer of features~(commonly utilized to compute OOD scores).   
    Our results demonstrate that the training criterion is a crucial factor in the diversity of the models. 
        As shown in Fig.~\ref{fig:coupling}, the two models obtained from the same criterion training, their OOD's feature representations are highly correlated in the sense of optimal transport, indicating less disagreement on OOD samples.
    To further substantiate our findings, we also evaluated the loss barrier~\cite{frankle2020linear} between models trained on different criteria. 
            Our results demonstrate that the models trained using different criteria exhibit a more significant loss barrier, implying that the models do not have the same loss landscapes. Consequently, these models display greater dissimilarities.

Building on the aforementioned assumptions and findings, we devised a novel ensemble scheme that integrates models trained on different criteria but with the same structure and training data. 
    Our experiments show that this ensemble scheme outperforms other approaches, such as data-level k-fold ensembles~\cite{li2021kfolden}.
        Further, to reduce the computational overhead in the inference phase, we explored whether an OOD-sensitive network could be trained or distilled by aligning such ensemble's feature space that is more sensitive to OOD data.

\textbf{Contributions.} We make the following contributions:

\begin{itemize}
    \item We reveal that the previous ensembles' lack of success in detecting OOD samples can be attributed to the inadequate degree of diversity among models trained using the same criterion.
    \item We design a feature-level ensemble scheme that exploits the diversity of models based on different criterions, making the OOD samples more distant from the class center in average.
    %\item We propose to obtain more easily deployable OOD-sensitive models by distillation with ensemble for feature alignment.
    %这最后一点contribution和前面不衔接，而且有人提过了
\end{itemize}

\begin{figure}[t]
    \centering
    \includegraphics{_fig/coupling-matrix.pdf}
    \caption{Coupling matrix of the OOD sample penultimate layer feature distribution's Wasserstein distance of the two networks. Highlighting on the diagonal indicates that the two sets of feature representations are aligned relative to the sample, which indicates that there is little variability in the two distributions. SupCE = Supervised Cross  Entropy loss, SupCon = Supervised Contrastive loss~\cite{khosla2020supervised}, SimCLR = Simple Contrastive Learning Representation~\cite{chen2020simple}}
    \label{fig:coupling}
\end{figure}

==> _hist/1_Introduction_v3.tex <==
\section{Introduction}
State-of-the-art neural network models often exhibit overconfidence in their predictions due to their training and generalization in a static and closed environment. 
    Specifically, these models assume that the distribution of test samples is identical to that of the training samples. 
        However, in the open world, this assumption may not hold, as out-of-distribution (OOD) samples can arise from unreliable data sources or adversarial attacks. 
            Such OOD samples can introduce significant challenges to the generalization performance of these models.
Due to concerns related to reliability and safety, it is crucial to identify when input data is OOD. 
    Significant research efforts have been devoted to the detection of OOD samples~\cite{liang2018enhancing,hendrycks2019using,ren2019likelihood,huang2021importance}, as well as the estimation of uncertainty~\cite{lakshminarayanan2017simple} in networks.

In practice, researchers propose employing an ensemble of neural networks, which involves combining multiple independent models to enhance the robustness of model predictions against OOD samples~\cite{lakshminarayanan2017simple,zaidi2021neural,Malinin2020Ensemble,kariyappa2021protecting,li2021kfolden,xue2022boosting,ding2022hyperparameter}. 
Inspired by the Bagging~\cite{breiman1996bagging}, researchers have proposed \emph{Deep Ensembles}~\cite{lakshminarayanan2017simple}, which calculate the average of the posterior probabilities generated by multiple models with different initializations. 
    This approach offers the advantages of being both pervasive and scalable. 

    %However, ensembles face two main challenges. 
    %The first 
  %  The first is related to the intrinsic mode connectivity~\cite{pagliardini2022agree,frankle2020linear} of neural networks. 
  %      Specifically, the members of an ensemble tend to exhibit strong consistency, meaning that even with different initializations and training samples, the resulting models map input samples to similar posterior distributions after training with the same criterion.
            %The second issue with ensembles is that their computational overhead increases significantly with the number of ensemble members, which can limit their deployment on real-world edge devices with limited resources and real-time requirements. Although ensembles are effective, this overhead can make them unsuitable for certain applications.
            
However, recent work~\cite{abe2022deep} claims that the ensemble diversity does not meaningfully contribute to a \emph{Deep Ensemble's} OOD detection performance improvement. 
    This means that \emph{Deep Ensemble's} performance is consistent with that of a single model of equivalent size.
        We observe this phenomenon and attribute it to the fact that the diversity provided by naive \emph{Deep Ensemble} through different model initializations is not significant enough.
     Specifically, the individuals in an naive ensemble tend to exhibit strong consistency in feature representation.
        This feature representation level consistency is because individuals' comprehension of data distribution in an ensemble model are highly similar, due to intrinsic mode connectivity~\cite{pagliardini2022agree,frankle2020linear,ainsworth2023git} among neural networks.


From feature representation perspective, we experimentally reveals that neural networks trained with same loss but with different initializations and stochastic gradient descent (SGD) display only weak differences in their encoding of the same input in the representation space.
    To achieve this, we employed the Optimal Transport  and its corresponding sample coupling matrix along with Self-Coupling Index to quantify the differences in the distribution of the same dataset's encoding by various models in the penultimate layer of features~(commonly utilized to compute OOD scores).   

From loss landscape perspective, we theoretically reveals that the above feature representation consistency arises from the hypothesis that, given the training criterion, the neural network loss landscapes, accounting for various possible permutation symmetries, comprises only a single loss basin~\cite{ainsworth2023git}. 
        Consequently, networks trained on the same distributed dataset with the same criterion using SGD are highly correlated or even functionally equivalent. 
            We find a correlation between the two models' loss barrier and the Self-Coupling Index between their feature representations.
                This marginal disparity impedes the ensemble's ability to achieve anticipated outcomes in detecting OOD.
%Our study, conducted through a combination of experimental and theoretical analyses, 

Based on feature representation and loss landscape perspective findings and assumptions, we demonstrate that the training task is a crucial factor in the diversity of the models. 
    Individual models in ensemble develop their different comprehension of the data in different training tasks. 
        As shown in Fig.~\ref{fig:coupling}, models using the same training task have a highly similar comprehension of data formation at the feature representation level, and vice versa.
%Experimentally and theoretically, we reveals that neural networks trained using the same criterion but with different initializations and stochastic gradient descent (SGD) display only weak differences in their encoding of the same input in the representation space.
 %   This phenomenon arises from the hypothesis that, given the training criterion, the approximation of the neural network loss landscapes, accounting for various possible permutation symmetries, comprises only a single loss basin. \cite{ainsworth2023git}
  %      Consequently, networks trained on the same distributed dataset with the same criterion using SGD are highly correlated or even functionally equivalent to a considerable extent. 
%Nonetheless, this marginal disparity impedes the ensemble's ability to achieve anticipated outcomes in detecting OOD samples.
%In this paper, we employed the Wasserstein distance and its corresponding sample coupling matrix to quantify the differences in the distribution of the same dataset's encoding by various models in the penultimate layer of features~(commonly utilized to compute OOD scores).   
   % Our results demonstrate that the training criterion is a crucial factor in the diversity of the models. 
      %  As shown in Fig.~\ref{fig:coupling}, the two models obtained from the same criterion training, their OOD's feature representations are highly correlated in the sense of optimal transport, indicating less disagreement on OOD samples.
  %  To further substantiate our findings, we also evaluated the loss barrier~\cite{frankle2020linear} between models trained on different criteria. 
       %     Our results demonstrate that the models trained using different criteria exhibit a more significant loss barrier, implying that the models do not have the same loss landscapes. Consequently, these models display greater dissimilarities.
Therefore, considering the diversity of model's comprehension, we devised a novel ensemble scheme, named Multi-Comprehension Ensemble~(MC Ensmble) that integrates models trained on different task but with the same structure and training data. 
%Building on the aforementioned assumptions and findings, we devised a novel ensemble scheme that integrates models trained on different criteria but with the same structure and training data. 
    Our experiments show that this ensemble scheme outperforms other ensemble approaches on CIFAR10 and Imagenet Benchmarks.
       % Further, to reduce the computational overhead in the inference phase, we explored whether an OOD-sensitive network could be trained or distilled by aligning such ensemble's feature space that is more sensitive to OOD data.

\textbf{Contributions.} We make the following contributions:

\begin{itemize}
    \item We reveal that the previous ensembles' lack of success in detecting OOD samples can be attributed to the inadequate degree of diversity among models trained using the same criterion.
    \item We design a feature-level ensemble scheme that exploits the diversity of models based on different criterions, making the OOD samples more distant from the class center in average.
    %\item We propose to obtain more easily deployable OOD-sensitive models by distillation with ensemble for feature alignment.
    %这最后一点contribution和前面不衔接，而且有人提过了
\end{itemize}

\begin{figure}[t]
    \centering
    \includegraphics{_fig/coupling-matrix.pdf}
    \caption{Coupling matrix of the OOD sample penultimate layer feature distribution's Wasserstein distance of the two networks. Highlighting on the diagonal indicates that the two sets of feature representations are aligned relative to the sample, which indicates that there is little variability in the two distributions. SupCE = Supervised Cross  Entropy loss, SupCon = Supervised Contrastive loss~\cite{khosla2020supervised}, SimCLR = Simple Contrastive Learning Representation~\cite{chen2020simple}}
    \label{fig:coupling}
\end{figure}

==> _hist/2_Background.tex <==
Usually a neural network can be divided into two parts in the inference phase, the encoder $g(\cdot)$ that encodes the input into the representation space and the functional projection head $h(\cdot)$~(i.e. classification head).

The OOD detection problem can be transformed into a 0-1 classification problem, where positive examples represent OOD and negative examples represent ID. The reason why an ensemble works in OOD detection is based on the followin bias-variance decomposition for 0-1 classification:
\begin{equation}
    Error(C) = \sum_{x}P(x)(bias^2[f_{ensemble}(x)]+ var[f_{ensemble}(x)]+\sigma^2(x))
\end{equation}

%\frac{1}{M^2}\sum_{i=1}^{M}var(f_i(x))+\frac{1}{M(M-1)}\sum_{i \neq j}cov(f_i(x),f_j(x))+

==> _hist/2_Background_v1.tex <==

\section{Why Model Diversity Matters in OOD Detection Ensemble?}

Let $\mathcal{X}$ and $\mathcal{Y}$ be the input space and label space. 
    We define the penultimate layer representation space of the neural network as $\mathcal{R}$. 
Then the neural network trained on hypothesis $H$ can be represented as $f_H(x) = h_H(g_H(x)), x\in\mathcal{X} $, where $g_H: \mathcal{X} \to \mathcal{R}$ is the feature encoder and $h_H: \mathcal{R} \to \mathcal{Y}$ is the projection head. 
    The hypothesis $H$ contains the training criterion (i.e. Cross-entropy loss, SimCLR~\cite{chen2020simple}, SupCon loss~\cite{khosla2020supervised}), data distribution $D$, initialization $\Theta$, and other training configuration.

\begin{figure*}[t]
    \centering
    \includegraphics{_fig/loss basin1.pdf}
    \caption{(a)~Models trained by \textbf{different initialization} ($\Theta_1$, $\Theta_2$) but with the same cross-entropy classification task (\textit{CE-SGD}) can fall into the same or symmetric loss basin, which can be affine-transformed into the same basin (\textit{Re-Basin}~\cite{ainsworth2023git}). This indicates the two models provide little variability. (b)~By contrast, a \textbf{different comprehension task} (\textit{SimCLR-SGD}) directs the model parameters in other directions. When \textit{SimCLR-SGD} model weights are relocated to the same loss landscape of \textit{CE-SGD} weights, we can observe the loss barrier between two sets of weights is high so that \textit{Re-Basin} is not possible, thus increasing the model and feature diversity. }
    \label{fig:rebasin}
\end{figure*}  

\subsection{Out-of-distribution Detection}


We consider the OOD detection task as a 0-1 classification problem on an open set, where samples sampled from a distribution consistent with the training set $D_{train}$ (ID) are regarded as positive, and samples sampled from outside the distribution (OOD) are regarded as negative (assumed to be sampled from $D_{OOD}$).
    A simple and common OOD detection method is to score the feature representation $z = g_H(x) \in \mathcal{R}$ in the penultimate layer space based on the scoring metrics $s(z) \in \mathbb{R}$~\cite{liu2020energy,sun2022out,liang2018enhancing}. 
        Then we determine the sample by its score and a threshold $\tau$ that the sample is ID if $s(z)>\tau$ and vice versa OOD. The probability that an OOD detector coupled with a neural network trained on hypothesis $H$ regard sample $x$ as positive can be formulated as:
\begin{equation}
 \resizebox{0.91\hsize}{!}{$
    P(Y_H = 1 |x) = E[\mathbf{1}[s(g_H(x))>\tau]] = P(s(g_H(x))>\tau)    $}
\end{equation}
\begin{comment}
\begin{equation}
    \Phi_H(x,\tau) = \left\{\begin{array}{lr}
        1, & if\ s(g_H(x))>\tau \\
        0, & if\ s(g_H(x))<\tau
    \end{array}
    \right.
\end{equation}
\end{comment}
            %Thus, the OOD detection performance is determined mainly by the performance of feature encoder and scoring metric.

Regarded as a 0-1 classification problem, the loss of detector $\Phi_H$ can be subjected to a bias-variance decomposition~\cite{kohavi1996bias} like Eq.~\ref{equ: composition}, see Appendix A.1 for proof.
\begin{equation}
 \resizebox{0.91\hsize}{!}{$
\begin{split}
    \mathcal{L}(\Phi_H) &= \frac{1}{2}\sum_x P(x)[\underbrace{\sum_{y=0}^1(P(\Phi_H=y|x)-P(\Phi_T = y|x))^2}_{bias^2_H}\\
    &+\underbrace{(1-\sum_{y=0}^1P(\Phi_H=y|x)^2)}_{variance_H}+\sigma_x^2]
    %(\sigma_x^2 + bias^2 + variance)
        \label{equ: composition}
\end{split}$}
\end{equation}
where $T$ means ground truth hypothesis which can be seen as a perfect OOD detector and $\sigma_x^2 = 1- \sum_{y=0}^1P(Y_T=y|x)^2$ is an irreducible error.

\subsection{Diversity in Ensemble Learning}

The ensemble is widely used in the deep learning community as a scalable and simple method. 
% bias of the ensemble equals the expectation of individual bias and the
    The core idea of the ensemble is to exploit the diversity among different models. The variance of an ensemble in Eq.~\ref{equ: composition} with $M$ individuals which are based on hypothesis $H_i, i \in \{1, \cdots, M\}$ can be further composed to:
%\begin{equation}
%    bias_{ens} = \frac{1}{M} \sum_{i=1}^M bias_{H_i}
%\end{equation}
\begin{equation}
 \resizebox{0.91\hsize}{!}{$
\begin{split}
    &variance_{ens} = \frac{1}{M}[\underbrace{\frac{1}{M}\sum_{i=1}^{M}(1-\sum_{y=0}^1P(\Phi_{H_i}=y|x)^2)}_{E[variance_{H_i}]}\\
    &+\underbrace{\frac{1}{M}\sum_{i=1}^{M}\sum_{j \neq i}(1-\sum_{y=0}^1P(\Phi_{H_i}=y|x)P(\Phi_{H_j}=y|x))}_{covariance}],
    \end{split}$}
\end{equation}
hence, the variance of an ensemble can be bounded by a lower boundary $\frac{1}{M}E[variance_{H_i}]$ and an upper boundary $E[variance_{H_i}]$. See Appendix A.1 for proof.
    When the $covariance$ is 0, i.e., all detectors are completely uncorrelated, the variance of the ensemble can reach the lower bound, which is $\frac{1}{M}$ in a single model; 
        while when all models are highly similar, the covariance of the models will become larger and the significance of the ensemble will then diminish.
    Therefore, substantial model diversity can significantly reduce the covariance term, thus improving the ensemble performance.


==> _txt/0_Abstract_v3.tex <==
\begin{abstract}
Recent research underscores the pivotal role of the Out-of-Distribution (OOD) feature representation field scale in determining the efficacy of models in OOD detection. Consequently, the adoption of model ensembles has emerged as a prominent strategy to augment this feature representation field, capitalizing on anticipated model diversity.

However, our introduction of novel qualitative and quantitative model ensemble evaluation methods, specifically Loss Basin/Barrier Visualization and the Self-Coupling Index, reveals a critical drawback in existing ensemble methods. We find that these methods incorporate weights that are affine-transformable, exhibiting limited variability and thus failing to achieve the desired diversity in feature representation.

To address this limitation, we elevate the dimensions of traditional model ensembles, incorporating various factors such as different weight initializations, data holdout, etc., into distinct supervision tasks. This innovative approach, termed Multi-Comprehension (MC) Ensemble, leverages diverse training tasks to generate distinct comprehensions of the data and labels, thereby extending the feature representation field.

Our experimental results demonstrate the superior performance of the MC Ensemble strategy in OOD detection compared to both the naive Deep Ensemble method and a standalone model of comparable size. This underscores the effectiveness of our proposed approach in enhancing the model's capability to detect instances outside its training distribution.
\end{abstract}


==> _txt/9_Rebuttal.tex <==
\section{Rebuttal}
\subsection{General Response}

Dear Area Chair and Reviewers,

We appreciate reviewers' precious time and valuable advice. We are happy that most of reviewers acknowledged our motivation (16fL, nZyz), paper presentation (wBv7, Mibu, uVwC, nZyz), methods (wBv7, Mibu, uVwC, nZyz, 16fL) and experiments/analysis (wBv7, Mibu, uVwC, nZyz, 16fL). 

At the same time, we note the concerns and suggestions of the reviewers on our work. We provide extraordinary experiment results and detailed answers to all the questions raised by the reviewers in the following individual responses. We hope these responses address your questions and concerns well. If you still have questions and concerns, we appreciate you discussing them further with us!


Since NeurIPS 2023 does not allow for the submission of revised papers at the rebuttal stage, we are committed to incorporating changes based on the comments of the reviewers in subsequent revised release. 


We thank the reviewers (wBv7, nZyz, 16fL) for reminding us that we should include a separate section on limitations and broader impacts. We will add two sections to discuss limitations and broader impact in revised paper as follows.


8 Limitations

This paper proposes to aggregate multiple models trained with different tasks to form a multi-comprehension ensemble for better OOD detection performance. The limitation of this paper can be that: (1) In current work, the task/criteria pool we have explored cannot be described as large, and this makes it possible for us to miss the opportunity to find a more powerful MC ensemble. As more and more training task/criteria being proposed, the task/criteria pool need further study. (2) The computation overhead of MC Ensemble is still $M\times$ compared to single standalone model with same backbone. In the case of constrained computation resource, the latency may increase. 

9 Broader Impact

Generally, we believe OOD detection is an important component of AI safety. Enhancing OOD detection impacts the reliability of AI application in autonomous driving, healthcare, and others. The negative impact may be that the large amount of computation of ensemble-based model may cause larger computational resource footprint and carbon footprint.
\subsection{Reviewer nZyz}

We sincerely appreciate the constructive comments from reviewer nZyz and the time spent on reviewing this paper. We address the questions and clarify the issues accordingly as described below.

> **[Weakness 1]** : (minor) The most techniques the paper uses already exist (e.g. CE, SimCLR, SupCon). If this paper can propose better training methods based on the understanding of increasing model diversity, the results may be improved further.

**[Reply to W1]** : We verified that attempts to obtain diverse feature representations incorporating multi-comprehension using multiple losses training the same single model simultaneously failed. Multiple losses interfere with each other and eventually lead to convergence problems. To solve this problem of interference in training, we decided to use the method of training individual models independently and then averaging the penultimate layer of features. Meanwhile, the success of MC Ensemble distillation demonstrates that this capability by multi-comprehension diversity can be transferred to a single model, hinting at the possibility that there exists a straightforward training method for a single model to acquire this capability. The exploration of this approach we leave for future work. The novelty contribution to the community of this paper is that we validate the effectiveness of this multi-comprehension diversity.

> **[Weakness 2]** : In table 3, since MC Ens. leverages contrastive learning training, it's hard to compare MC Ens.+MSP, MC Ens.+Mahala., and MC Ens.+Energy. I suggest adding the following experiments to make the comparision easier: MSP+SimCLR, Energy+SimCLR, Mahala.+SimCLR, MSP+SupCon, Energy+SupCon, Mahala.+SupCon.

**[Reply to W2]** : Thank you for your suggestions. We conduct the experiments in Table 3 to evaluate the combinability of MC ensemble and commonly used OOD scoring metrics. We add the following experiments on CIFAR benchmark to address your concern.

|Training Task|Scoring Metric|SVHN||LSUN||iSUN||Texture||Place365||Average||
|-|-|-|-|-|-|-|-|-|-|-|-|-|-|
|||FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|
|SimCLR|MSP    |58.71|91.38|38.97|94.62|51.92|91.99|79.85|83.56|60.35|89.31|57.96|90.17|
|SimCLR|Mahala.|11.35|97.31|38.42|93.72|23.57|94.31|28.82|92.44|75.44|78.42|35.52|91.24|
|SimCLR|Energy |54.31|91.33|17.82|96.35|28.96|94.50|42.97|91.00|58.34|90.07|40.48|92.65|
|SimCLR|KNN    |41.69|92.07|29.68|93.44|43.60|91.60|32.98|92.77|38.41|91.72|29.27|94.62|
|SupCon|MSP    |63.24|88.57|52.94|89.98|50.04|91.72|69.85|85.09|70.31|85.65|61.27|88.20|
|SupCon|Mahala.|4.82|98.48|35.07|95.46|46.25|89.27|19.37|96.36|40.35|90.96|29.17|94.10|
|SupCon|Energy |44.35|91.03|13.11|97.45|24.65|95.51|26.71|93.94|43.26|89.18|30.41|93.42|
|SupCon|KNN    |2.42|99.52|1.78|99.48|20.06|96.74|8.09|98.56|23.02|95.36|11.07|97.93|
|MCEns.|MSP    |37.49|92.22|33.96|94.96|43.96|92.21|43.68|92.43|39.68|90.15|39.75|92.39|
|MCEns.|Mahala.|2.09|99.48|43.35|93.79|21.59|94.77|14.31|94.68|27.68|89.88|21.80|94.52| 
|MCEns.|Energy |34.99|92.58|6.05|99.05|17.96|96.59|23.97|91.92|33.02|92.37|23.20|94.50| 
|MCEns.|KNN|1.35|99.70|1.45|99.80|7.88|98.09|4.07|99.05|13.19|97.01|5.58|98.73|

> **[Weakness 3]** : The paper mentions many related concepts, e.g. Git Re-basin, Loss Barier, many existing ensemble methods. However, there is not a Related Work section to explain them.


**[Reply to W3]** : We will add a Related Work section in revised version as following.

2 Related Work

2.1 Loss Barrier

A loss barrier [13] between two models refers to a scenario where the optimization landscape, as defined by the loss function, presents a considerable and challenging obstacle for transitioning from one model to another. When attempting to move from one model to another, the goal is to adjust the parameters in a way that leads to improved performance on a specific task. However, if there exists a loss barrier between the two models, this means that making parameter updates to transition from the first model to the second model might involve encountering a region in the parameter space where the loss function increases significantly.

2.2 Git Rebasin

The postulate of Git Rebasin [2] methodology posits that a substantial subset of Stochastic Gradient Descent (SGD) solutions attained through the customary training regimen of neural networks belongs to a discernible collection, wherein the constituent elements can be systematically permuted. This permutation yields a configuration wherein no loss barrier in loss landscape exist along the trajectory of linear interpolation connecting any two permuted constituents.

2.3 Ensemble Learning

Ensemble methods have been a longstanding approach to enhancing model performance by combining the predictions of multiple models. Bagging [3] and Boosting [A1] are classic ensemble techniques that aim to mitigate overfitting and bias in predictions. Deep ensembles, as introduced by [23], leverage multiple neural networks with different initializations to capture model uncertainty and encourage diverse parameter sampling. SSLC[39] and kFolden [25] combined the traditional idea based on the difference in data samples with the data leave-out approach to construct deep ensembles. All of these ensembles have been effective in the OOD detection problem.

>**[Limitations]** : It seems that the paper does not have a limitation or negative societal impact section. 

**[Reply to Limitation]** : We will add a seperate limitations section and a broader impact section. Due to Author Response word limits, the specifics are in the general response.

**Reference**:
Due to Author Response word limits, we have listed here only the references that do not appear in the initial manuscript.
[A1] Freund, Yoav, and Robert E. Schapire. "Experiments with a new boosting algorithm." ICML. Vol. 96. 1996.



\subsection{Reviewer 16fL}

We sincerely appreciate the constructive comments from reviewer 16fL and the time spent on reviewing this paper. We address the questions and clarify the issues accordingly as described below.

> **[Weakness 1]**: The only concern is the innate problem of ensemble methods: computation. Although the authors have provided an additional distillation tactic to improve efficiency, there could be non-ensemble post-hoc OOD detection methods that are more efficient with comparable performance with MC ensemble. That being said, Table 3 could be more helpful if more recent post-hoc methods are provided for comparison. Latency comparison (other than number of parameters) with previous post-hoc methods could be useful as well.

**[Reply to W1]** : The components that contribute to the latency of the OOD detection method usually contain such two phases: (1) Generation of penultimate layer feature representations (2) Computation of out-of-distribution discriminant score.  

In the first phase, latency depends on the inference time of the backbone network. The computational overhead of an MC Ensemble consisting of $M$ individual models is $M\times $ that of a single model (we ignore the overhead of averaging feature, since it is negligibly small compared to neural network models). However, since these individual models are independent of each other, they are model-level parallelizable. Typically, in inference phases with sufficient computation resource, it is possible to achieve a high degree of parallelism of these individual models dies on a single device with the help of Nvidia's Multi-Process Scheduling (MPS) or Multi-Instance GPU (MIG) technology. For instance, we set three individual models (ResNet-18) as multiple independent processes, and utilized Nvidia MIG technology to let these models run simultaneously on the same A100 GPU, with batch size set to 16 (small batch size is more in line with real-world real-time reasoning needs), the latency of MC Ensemble to generate the penultimate layer features was 9.4 ms, while the single ResNet-18 model took 9.3 ms. In this case, MC ensemble can even achieve faster inference than some standalone models of the same size. For example, ResNet-62, which is the same size as MC Ensemble, took 17.0 ms because of deeper architecture.

In the second phase, latency depends on the OOD scoring methods. Since MC ensemble can be used with any kind of OOD discriminant scoring metric, it does not have any computational difference in latency compared to other post-hoc OOD detection methods if we use same scoring metric. With the hyperparameters determined, the computational complexity of the OOD discriminant score depends only on the dimensions of the features, and our strategy of using feature average ensures that the feature dimensions are invariant compared to the original backbone network. Therefore the second phase computational latency depends only on which OOD scoring metric is combined with the MC Ensemble. 



Performance comparison with more recent methods are provided below:

|Method|Venue|SVHN||LSUN||iSUN||Texture||Place365||Average||
|-|-|-|-|-|-|-|-|-|-|-|-|-|-|
|||FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|
|FeatureNorm|CVPR2023|7.13|98.65|27.08|95.25|26.02|95.38|31.18|92.31|62.54|84.62|30.79|93.24|
|DOE*|ICLR2023|2.65|99.36|0|99.89|0.75|99.67|7.25|98.47|15.10|96.53|5.15|98.78|
|CIDER|ICLR2023|3.04|99.50|4.10|99.14|15.94|97.10|13.19|97.39|26.60|94.64|12.57|97.55|
|ReAct|NeurIPS2021|49.77|92.18|17.94|96.98|20.84|96.46|47.96|91.55|43.97|91.33|36.10|93.70|
|SHE|ICLR2023|5.87|98.74|6.67|98.42|4.16|98.85|-|-|6.31|98.70|-|-|
|DICE|ECCV2022|25.99|95.90|3.91|99.20|4.36|99.14|41.90|88.18|48.59|89.11|24.95|94.30|
|ASH-S|ICLR2023|6.51|98.56|4.96|98.92|5.17|98.90|24.34|95.09|48.45|88.31|17.89|95.96|
|BATS|NeurIPS2022|38.42|93.53|19.85|96.59|-|-|43.81|92.32|-|-|-|-|
|Watermark|NeurIPS2022|16.45|97.11|16.85|96.97|16.20|96.97|32.60|93.14|36.25|91.87|23.69|95.21|
|MCEns| Ours|1.35| 99.70| 1.45 |99.80| 7.88| 98.09 |4.07 |99.05 |13.19 |97.01 |5.58 |98.73|

*: Outlier Exposure based model. These models often perform well on benchmark but with limited generalization ability.

> **[Question 1]** : Judging from Table 8~10 in the supplement, it seems that the authors considered more tasks/criteria for MC ensemble. Was there a reason why the authors selected only 3 (SupCE, SupCon, SimCLR)? What happens if M = 2, 4, 5 etc.. were selected?


**[Reply to Q1]** In Section 6, we report the performance when $M = 2$. When $M = 3$, we first consider SupCon as first individual model because some works (SSD+ and KNN+) have revealed SupCon's excellent performance on OOD detection, and then SupCE and SimCLR are selected based on Eq.6. According to Eq.6, when $M = 4$, MOCO should be seleceted to participate the MC Ensemble, and when $M = 5$, JigClu should be added into MC Ensemble. The performance is as below: 
|M|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|
|-|-|-|-|-|-|-|-|-|-|-|-|-|
|3|1.35| 99.70| 1.45 |99.80| 7.88| 98.09 |4.07 |99.05 |13.19 |97.01 |5.58 |98.73|
|4|1.41|99.71|1.62|99.64|8.12|97.93|4.27|99.01|11.98|97.31|5.48|98.72|
|5|2.69|99.44|1.37|99.83|7.95|97.99|6.35|98.65|14.97|96.35|6.66|98.45|

>**[Question 2]** : As mentioned in the weakness section, how does OOD detection inference latency of MC Ensemble (and MC Ensemble with distillation) compare with previous post-hoc detection methods?

**[Reply to Q2]** : See reply to weakness 1.

>**[Question 3]** : (minor) L292 Tbale -> Table

**[Reply to Q3]** : We will fix that typo in revised version.

>**[Limitation]** : I do not see a separate limitations section. Please add a "limitations" section and a "broader impact" section.

**[Reply to Limitation]** : We will add a seperate limitations section and a broader impact section. Due to rebuttal word limits, the specifics are in the general response.

8 Limitations

This paper proposes to aggregate multiple models trained with different tasks to form a multi-comprehension ensemble for better OOD detection performance. The limitation of this paper can be that: (1) In current work, the task/criteria pool we have explored cannot be described as large, and this makes it possible for us to miss the opportunity to find a more powerful MC ensemble. As more and more training task/criteria being proposed, the task/criteria pool need further study. (2) The computation overhead of MC Ensemble is still $M\times$ compared to single standalone model with same backbone. In the case of constrained computation resource, the latency may increase. 

9 Broader Impact

Generally, we believe OOD detection is an important component of AI safety. Enhancing OOD detection impacts the reliability of AI application in autonomous driving, healthcare, and others. The negative impact may be that the large amount of computation of ensemble-based model may cause larger computational resource footprint and carbon footprint.

\subsection{Reviewer uVwc}

We sincerely appreciate the constructive comments from reviewer uVwc and the time spent on reviewing this paper. We address the questions and clarify the issues accordingly as described below.

> **[Weakness 1]** : The experiments conducted by the authors seem to be not comprehensive enough. In particular, the datasets span over two benchmarks: CIFAR and ImageNet, which may not authentically reveal the real-world application scenarios. The authors should consider involving more various datasets to further showcase the superiority of their method.

**[Reply to W1]** : CIFAR and ImageNet Benchmark are mostly used benchmarks in out-of-distribution detection community. As far as we know, most state-of-the-art general OOD detection methods [1-8] are evaluated on such two benchmarks. The two benchmarks were carefully designed to include both regular OOD problems (CIFAR vs 5 datasets) and more challenging near-OOD problems (CIFAR10 vs CIFAR100), as well as larger datasets (ImageNet Benchmark). We acknowledge that CIFAR and ImageNet are not the most up-to-date and realistic datasets in computer vision. But building a brand new OOD detection benchmark/dataset requires the efforts of the entire OOD community, which is beyond the scope of this paper.

> **[Weakness 2-1]** : The baselines used in this paper seem to be relatively outdated. In specific, most baselines are proposed before 2020, which cannot faithfully justify the superior performance of the proposed method.

**[Reply to W2-1]** : The comparison with mre recent model on CIFAR benchmark is provided as following:

|Method|Venue|SVHN||LSUN||iSUN||Texture||Place365||Average||
|-|-|-|-|-|-|-|-|-|-|-|-|-|-|
|||FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|FPR95|AUROC|
|FeatureNorm|CVPR2023|7.13|98.65|27.08|95.25|26.02|95.38|31.18|92.31|62.54|84.62|30.79|93.24|
|DOE*|ICLR2023|2.65|99.36|0|99.89|0.75|99.67|7.25|98.47|15.10|96.53|5.15|98.78|
|CIDER|ICLR2023|3.04|99.50|4.10|99.14|15.94|97.10|13.19|97.39|26.60|94.64|12.57|97.55|
|ReAct|NeurIPS2021|49.77|92.18|17.94|96.98|20.84|96.46|47.96|91.55|43.97|91.33|36.10|93.70|
|SHE|ICLR2023|5.87|98.74|6.67|98.42|4.16|98.85|-|-|6.31|98.70|-|-|
|DICE|ECCV2022|25.99|95.90|3.91|99.20|4.36|99.14|41.90|88.18|48.59|89.11|24.95|94.30|
|ASH-S|ICLR2023|6.51|98.56|4.96|98.92|5.17|98.90|24.34|95.09|48.45|88.31|17.89|95.96|
|BATS|NeurIPS2022|38.42|93.53|19.85|96.59|-|-|43.81|92.32|-|-|-|-|
|Watermark|NeurIPS2022|16.45|97.11|16.85|96.97|16.20|96.97|32.60|93.14|36.25|91.87|23.69|95.21|
|MCEns| Ours|1.35| 99.70| 1.45 |99.80| 7.88| 98.09 |4.07 |99.05 |13.19 |97.01 |5.58 |98.73|

*: Outlier Exposure based model. These models often perform well on benchmark but with limited generalization ability.

> **[Weakness 2-2]** : Moreover, the authors claim that KNN is a non-parameter approach, however, the reference seems to be a deep model that should involve training on parameters.

**[Reply to W2-2]** : Typically the OOD detection task consists of two phases, the backbone deep network that is shared with the main task, and the scoring metric that discriminates the OOD data. KNN in [7] is a non-parameter scoring metric acting on the feature representation generated by a deep model.

> **[Weakness 3]** : The authors provide a link to the code, however, nothing exists there.

**[Reply to W3]** : We fixed this issue and the code is now visible.

> **[Weakness 4]** : The authors mainly compare their method with baselines on the evaluation metrics regarding the performance. However, the experiments lack the necessary case studies or other qualitative analyses to showcase the intuition behind their method, i.e., why the method works. The ablation study seems not enough for justification.

**[Reply to W4]** : Our intuition behind this method is that ensemble diversity from multi-task/comprehension can boost OOD detection. Comparisons in Table 4,5,6 directly reveal the effectiveness of multi-comprehension against single-comprehension. The analysis regarding why this method works is in Section 2 and 3, where we justify our intuition with loss landscape and feature self-coupling, and Fig.1 and 2, Table 2 measure and visualize them. Ablation study in this work mainly focus on analysis what role's the contrastive learning, model scale play in OOD detection.

> **[Weakness 5]** : The usage of backbone ResNet18 should be reconsidered, as the larger backbones such as ViT generally exhibit better performance and requires fair comparisons.

**[Reply to W5]** : We report our OOD experiment result and self-coupling index on ResNet50 and ViT backbone networks in Section 5.2, Appendix A.3, A.4, A.6 and A.7. As ResNet18 is commonly used in OOD detection, for fair comparison, we still use ResNet18 as standard backbone on CIFAR benchmark. We acknowledge that stronger backbone networks will have stronger OOD performance, as shown in [9].

> **[Question and Limitation]** : See reply to W5, W4 and W2 respectively.


[1] Wang, Qizhou, et al. "Out-of-distribution Detection with Implicit Outlier Transformation." ICLR. 2023.
[2] Ming, Yifei, et al. "How to Exploit Hyperspherical Embeddings for Out-of-Distribution Detection?." ICLR. 2023.
[3] Zhang, Jinsong, et al. "Out-of-Distribution Detection based on In-Distribution Data Patterns Memorization with Modern Hopfield Energy." ICLR. 2023.
[4] Djurisic, Andrija, et al. "Extremely Simple Activation Shaping for Out-of-Distribution Detection." ICLR. 2023.
[5] Zhu, Yao, et al. "Boosting Out-of-distribution Detection with Typical Features." NeurIPS. 2022.
[6] Wang, Qizhou, et al. "Watermarking for Out-of-distribution Detection." NeurIPS. 2022.
[7] Sun, Yiyou, et al. "Out-of-distribution detection with deep nearest neighbors." ICML. 2022. 
[8] Sehwag, Vikash, et al. "SSD: A Unified Framework for Self-Supervised Outlier Detection." ICLR. 2021.
[9] Fort, Stanislav. et al. "Exploring the limits of out-of-distribution detection." NeurIPS. 2021.

\subsection{Reviewer Mibu}

We sincerely appreciate the constructive comments from reviewer Mibu and the time spent on reviewing this paper. We address the questions and clarify the issues accordingly as described below.

> **[W1]**: The authors use Loss Barrier to evaluate linear connectivity and vividly show this process in Figure 1. But specifically, how large of a Barrier might cause linear disconnection? Is the Re-Basin available area in Figure 1 actually measured, or just schematic? In other words, is Figure 1 a realistic diagram or a schematic diagram? 

**[Reply to W1]** : There is no commonly accepted threshold for the loss barrier that causes linear disconnection; in practice this value can be set at $0\sim0.2 \times$ the loss at random initialization. Figure 1 is a partial capture of a real loss landscape. Parameters in Basin 1 and Basin 2 can be transformed to each other by a permutation, in other word, it's a realistic diagram. But the green ellipse marked with a dotted line is just for schematic purposes, indicating Basin 1 and 2 are Re-Basin available, while Basin 3 is not.

> **[W2-1]**: The authors claim that SupCE and SimCLR are linearly disconnected and propose SCI and Loss Barrier to support this view, which is also the premise of their proposed method. But SimCLR actually has excellent linear probing performance, reaching 95.3% performance on CIFAR10 and 80.2% accuracy on CIFAR100. In my view, the linear probing performance of self-supervised methods is able to reflect their linear connectivity with SupCE. Therefore, this seems to contradict the view of this paper.

**[Reply to W2-1]** : Although SimCLR has excellent linear probing performance, it doesn't necessarily indicate the linear connectivity with SupCE. This is because there are multiple local minimum in the loss landscape w.r.t parameter space [1], while some of the local minimum are mode connected after a simple permutation (symmetric/rotation/swap dimensions) while others are not. SimCLR and SupCE eventually bring the parameters into different local minimum that can not be connected by such permutation, indicating less linear connectivity in parameter space. Meanwhile, both SimCLR (with a linear probing head) and SupCE arrive a local minimum in loss landscape, which means both can achieve good performance on the main task (classification). That is saying, linear mode disconnection does not conflict with a good linear probing performance.

> **[W2-2]**: Secondly, Masked Image Modeling (MIM) methods represented by MAE usually have significantly worse linear probing performance than contrastive learning. If MIM is introduced in the MC Ensemble, can it achieve better results? 

**[Reply to W2-2]** The answer is yes. In Appendix A.6 and Table 14, we construct a ViT MC Ensemble, in which MAE is considered as an individual model, and we noticed a performance gain. We also measure the Self-Coupling Index between MAE and other training tasks as shown in Appendix A.3 and Table 11. A paper [2] made public after we completed this manuscript submission shows the role of MIM in OOD detection. We confirmed the effectiveness of their method and MIM in OOD detection in our follow-up experiments, and we will continue to focus on the role of MIM in MC Ensemble in our subsequent work. Thank you for your suggestions.

> **[W3]**: The authors use various scoring methods to compare with existing methods in the Table 3, showing their superiority. But should the authors compare with existing methods more fairly on the same scoring method? For example, MC Ens. + Mahala. should be used to compare with SSD+, which uses Mahala. Under such a comparison, is there a large performance difference between the proposed method and the existing methods? (e.g. The AUROC on the LSUN dataset is 4.69% behind.) 

**[Reply to W3]** : For fair comparison, we did the following experiments to verify the OOD performance (FPR95/AUROC) of MC ensemble with multiple scoring metrics. Mahala. Distance scoring metric used in SSD+ is cluster conditioned and few-shot OOD data boosted, thus directly comparing MCEns.+Mahala. with SSD+ will cause a unfair comparison.

|Scoring Metric|Training Task|SVHN||LSUN||iSUN||Texture||Place365||Average||
|-|-|-|-|-|-|-|-|-|-|-|-|-|-|
|Mahala.|SimCLR|11.35|97.31|38.42|93.72|23.57|94.31|28.82|92.44|75.44|78.42|35.52|91.24|
|Mahala.|SupCon|4.82|98.48|35.07|95.46|46.25|89.27|19.37|96.36|40.35|90.96|29.17|94.10|
|Mahala.|MCEns.|2.09|99.48|43.35|93.79|21.59|94.77|14.31|94.68|27.68|89.88|21.80|94.52| 
|Energy |SimCLR|54.31|91.33|17.82|96.35|28.96|94.50|42.97|91.00|58.34|90.07|40.48|92.65|
|Energy |SupCon|44.35|91.03|13.11|97.45|24.65|95.51|26.71|93.94|43.26|89.18|30.41|93.42|
|Energy |MCEns.|34.99|92.58|6.05|99.05|17.96|96.59|23.97|91.92|33.02|92.37|23.20|94.50| 
|KNN   |SimCLR |41.69|92.07|29.68|93.44|43.60|91.60|32.98|92.77|38.41|91.72|29.27|94.62|
|KNN   |SupCon|2.42|99.52|1.78|99.48|20.06|96.74|8.09|98.56|23.02|95.36|11.07|97.93|
|KNN   |MCEns.|1.35|99.70|1.45|99.80|7.88|98.09|4.07|99.05|13.19|97.01|5.58|98.73|
|SSD+|- |1.51|99.68|6.09|98.48|33.60|95.16|12.98|97.70|28.41|94.72|16.52|97.15|
|Mahala.(SSD+)|MCEns.|1.57|99.60|3.25|99.35|15.59|96.77|14.32|96.98|21.68|96.12|10.28|97.76| 

> **[Q1]**: Did the authors use formula 6 to select the optimal hypotheses? Can they provide more implementation details?

**[Reply to Q1]** : Yes, we use Eq.(6) for model selection. As shown in Appendix A.3, we measured SCI between 2 model sets in which model trained with different tasks, we take the first set as our model pool. As SupCon's excellent performance shown in SSD+ and KNN+, we take it as base individual model, then according to Eq.(6), SimCLR, SupCE, MOCO, JigClu, RoeNet are added in turn, as M increase from 2 to 6.



[1] Ainsworth, et al. "Git Re-Basin: Merging Models modulo Permutation Symmetries." ICLR. 2023.
[2] Li, Jingyao, et al. "Rethinking Out-of-distribution (OOD) Detection: Masked Image Modeling is All You Need." CVPR. 2023.

\subsection{Reviewer wBv7}

We sincerely appreciate the constructive comments from reviewer wBv7 and the time spent on reviewing this paper. We address the questions and clarify the issues accordingly as described below.

> **[Weakness 1]**: How is feature diversity related to OOD detection in principle? Reducing the variance doesn't necessarily improve OOD detection performance as the bias term (Eq (2)) can be significantly increased with a bad model in the ensemble.

**[Reply to W1]** :  Unlike traditional ensemble methods such as Bagging, Boosting, etc., deep enesmble has a basic assumption for each individual model: all models in the model pool should be well-trained so that there is no bad model leading to high bias. This ensures that no bad models are mixed into the ensemble. As shown in Table 4 and 6, all the basic individual models show not-bad OOD detection performance. But your concern is also right, when a bad model is added into ensemble, the bias term significantly increase. In fact, at the early stage in our experiment, our SimCLR model was not well-trained and we observe a significant performance drop in MC ensemble (with AUROC ~80%). Therefore, ensuring that all the individual model in the model pool/ensemble well-trained is critical to MC Ensemble.

> **[Weakness 2]**: The authors do not provide sufficient evidence why averaging the features of models trained with different losses do not counteract with each other. 

**[Reply to W2]** :  Averaging features will not lead to counteraction for the following reasons:
(1) The feature space is a high-dimensional space. In a higher dimensional space, arbitrary two vectors are almost orthogonal. This is based on the fact that, for a n-dim space, the angle $\theta$ between any two vectors satisfies: $P(|\theta-\frac{\pi}{2}|\leq m) = 1 - \frac{\int_{0}^{\frac{\pi}{2}-m}\sin^{n-2}\theta d\theta}{\int_{0}^{\frac{\pi}{2}}\sin^{n-2}\theta d\theta}$, where the numerator $\int_{0}^{\frac{\pi}{2}-m}\sin^{n-2}\theta d\theta < (\frac{\pi}{2}-m)\sin^{n-2}(\frac{\pi}{2}-m)$ decreases exponentially with $n$, while the denominator $\int_{0}^{\frac{\pi}{2}}\sin^{n-2}\theta d\theta > \frac{2\sqrt2}{3\sqrt{n-2}}$ decreases no faster than $o(\sqrt n)$. This suggests that any two features are almost orthogonal and that averaging them will not counteract each other.
(2) Our models are selected based on self-coupling index, which indicates that there is no affine transformation can calibrate features generated by those models for all samples. If such an counteraction happens, all class-conditional feature representations of a sample should be symmetrical to each other, which leading to the existence of a affine transformation between two representations, and thus the self-coupling index would be 1, against our assumption of low self-coupling index.

> **[Weakness 3]**: The writing of the paper can be further improved. Multiple notations and statements are used without definitions. 

**[Reply to W3]** : Thanks for pointing out the problems with the paper. In equation of Appendix L492 and L494, all the notations like $P(\Phi_H=y)(\Phi_T=y)$, $P(\Phi_H=y)-(\Phi_T=y)$and $(\Phi_T=y)^2$ should be corrected to $P(\Phi_H=y) P(\Phi_T=y)$, $P(\Phi_H=y)-P(\Phi_T=y)$ and $P(\Phi_T=y)^2$. We'll fix these in the revised paper.
In L106, the term "mode" refers to a local minimum in the loss landscape regarding parameter space of a neural network. Mode connectivity suggests that there might exist a continuous path $Pa(t)$ in parameter space that connects the two local minima. $Pa(t): \Theta_A = Pa(0) \rightarrow Pa(t) \rightarrow \Theta_b = Pa(1)$, where $t$ is a parameter that ranges from 0 to 1, and $Pa(t)$is a function that traces a path in the parameter space, and in this path the loss function should remain relatively low, meaning that the path smoothly transitions from one local minimum to the other.

> **[Question 1]**: In L493, "Due to the independence between the detector and ground truth, the first term disappears". A good OOD detector should be highly correlated with the ground truth classifier, so I doubt if the Eq (1) in L82 is correct.

**[Reply to Q1]** : 
Theorem: $\Theta_H$ and $\Theta_T$ are conditionally independent given target $f$ and a test point $x$.
Proof: $P(\Theta_T,\Theta_H|f,x)=P(\Theta_T|\Theta_H,f,x)P(\Theta_H|f,x)=P(\Theta_T|f,x)P(\Theta_H|f,x)$.
The last equality is true because by definition, the ground truth classifier $\Theta_T$ only depends on the target $f$ and the test point $x$.

> **[Question 2\&3]**: Can authors provide further clarification on why OOD detection risk Eq 2 can be decreased with MC ensemble? Why is the bias term not increased with models trained with different losses (see Weakness 1)? Can authors explain why feature level ensemble with models trained by different losses do not counteract each other (see Weakness 2)?

**[Reply to Q2\&3]** For the first question, the variance term of OOD risk decreases as the diversity of models increase while we control the bias term with well-trained model pool. See reply to W1 and W2.

> **[Question 4]** : Is ID classification accuracy included in the manuscript? If possible, can authors provide a table (or tables) including the ID accuracy with different ensemble strategies?

**[Reply to Q4]** : We trained 9 ResNet18 with different tasks, the ID accuracy is presented as following, Single model's accuracy is average accuracy of three models:

|Method|ID accuracy(%)|
|-|-|
|SupCE|92.89|
|SimCLR|92.11|
|SupCon|93.57|
|3*SupCE|94.01|
|3*SimCLR|93.35|
|3*SupCon|94.36|
|MCEns.|94.27|

> **[Question 5]** :  Can authors also train baseline methods with the same 80% training set and compare with OOD performance? How is ID accuracy impacted?

**[Reply to Q5]** : Deep models are mostly data-driven, decreasing training data will have a bad impact on their performance.
|Model|ID|FPR95|AUROC|
|-|-|-|-|
|1|89.07|51.66|85.31|
|2|87.63|52.99|84.72|
|3|89.21|51.70|85.27|

> **[Limitations]** : See general response.
\newpage

\begin{figure}[t]
    \centering
    \includegraphics{_fig/feature_visual.pdf}
    \caption{t-SNE visualization of penultimate layer features of SupCE, SupCon, SimCLR, MC Ensemble(average), while class 0-9 are ID classes (CIFAR10) and class 10 is OOD (CIFAR100).}
\end{figure} 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

